Does Nash Envy Immunity

The most popular stability notion in games should be Nash equilibrium under the rationality of players who maximize their own payoff individually. In contrast, in many scenarios, players can be (partly) irrational with some unpredictable factors. Hence a strategy profile can be more robust if it is resilient against certain irrational behaviors. In this paper, we propose a stability notion that is resilient against envy. A strategy profile is said to be envy-proof if each player cannot gain a competitive edge with respect to the change in utility over the other players by deviation. Together with Nash equilibrium and another stability notion called immunity, we show how these separate notions are related to each other, whether they exist in games, and whether and when a strategy profile satisfying these notions can be efficiently found. We answer these questions by starting with the general two player game and extend the discussion for the approximate stability and for the corresponding fault-tolerance notions in multi-player games.

==> headers.ec.tex <==
\usepackage[T1]{fontenc}
%\usepackage[margin=1in]{geometry}
%\usepackage{fullpage} \usepackage{amssymb,amsmath,amsthm,amsfonts}
\usepackage{amssymb,amsmath,amsfonts}
\usepackage{mathtools}
\usepackage{textcomp}
\usepackage[utf8]{inputenc}


\usepackage{xspace}
\usepackage[mathscr]{eucal}
\usepackage{color}
%\usepackage{subfigure}
\usepackage{graphicx}
%\usepackage{epstopdf}
%\usepackage{epsfig}

%\usepackage{algorithmic}
%algorithmic and algpseudocode is not compatible

\usepackage{tikz}
\usetikzlibrary{arrows,positioning,calc,shapes.symbols,shapes.callouts,patterns}


% Other useful math packages
\usepackage{nicefrac}
\usepackage{bm}
\usepackage{mathtools}

% Algorithm packages %marked since ec/ACM submission already use \usepackage[ruled]{algorithm2e}
%\usepackage{algorithm}
\usepackage{algpseudocode}
%algorithmic and algpseudocode is not compatible

% Allow footnotes in table/tabular
\usepackage{footnote}
\makesavenoteenv{tabular}
\makesavenoteenv{table}

%%%%%%%%%%%%%%% Draft Stuff: notes/todos %%%%%%%%%%%%%

\usepackage{ifdraft}
\ifdraft{
%% %%% TODO margin boxes
\newcommand{\NOTE}[1]{\textcolor[rgb]{0.1,0.6,.1}{NOTE: {#1}}}
\newcommand{\TODO}[1]{\textcolor[rgb]{1,0.5,.1}{{#1}}}

%% \newcounter{todos}
%% \setcounter{todos}{0}
\newcommand{\marginTODO}[1]{%
  \marginpar{%
    \framebox[0.9\marginparwidth][t]{%
      \parbox[t]{0.85\marginparwidth}{%
        \raggedright\scriptsize{#1}%
   }}}%
%%   \stepcounter{todos}%
}
}
{
\newcommand{\TODO}[1]{}
\newcommand{\NOTE}[1]{}
\newcommand{\marginTODO}[1]{}
}

\newcommand*{\tabbox}[2][t]{%
    \vspace{0pt}\parbox[#1][1.0\baselineskip]{\textwidth}{\strut#2\strut}}

%% To save/control space
\setlength{\topsep}{4pt}
% \usepackage[margin=1in]{geometry}
\usepackage{times}
% \usepackage[compact]{titlesec}
%% \usepackage{paralist}
%% \renewenvironment{itemize}{\begin{asparaitem}}{\end{asparaitem}}
%% \renewenvironment{enumerate}{\begin{asparaenum}}{\end{asparaenum}}
\newcommand{\uglyparagraph}[1]{\smallskip\noindent{\bf{#1}}}
\renewcommand{\paragraph}{\uglyparagraph}
\newcommand{\itemparagraph}[1]{\bigskip\paragraph{$\circ$~#1}}
% \usepackage{afterpage}
\usepackage{paralist}
\usepackage{enumitem}
\setlist[itemize]{leftmargin=*}
\setlist[enumerate]{leftmargin=*}


%%%%%%%%% hyperref %%%%%%%%%%%
%\usepackage[pdftex,final,bookmarks=true,pdfstartview=FitH,colorlinks,linkcolor=blue,filecolor=blue,citecolor=blue,urlcolor=blue]{hyperref}


%%%%%%%%%%% Environments %%%%%%%%%%%%%%%%%%%%%%

%\newtheorem{theorem}{Theorem}
\newtheorem{informalthm}{Theorem (Informal Statement)}
%\newtheorem{definition}{Definition}[section]
\newtheorem{observation}{Observation}
\newtheorem{assumption}{Assumption}
%\newtheorem{corollary}[theorem]{Corollary}
%\newtheorem{lemma}{Lemma}
\newtheorem{claim}{Claim}
%\newtheorem{remark}{Remark}

\newenvironment{proofsketch}{\noindent{{\em Proof sketch:~}}}{\hfill $\Box$ \smallbreak}
%\renewenvironment{proof}{\noindent{{\em Proof:~}}}{\hfill $\Box$ \smallbreak}
% \newenvironment{expt}{\begin{quotation}\noindent \vspace*{-18pt}}{\end{quotation}}
\newenvironment{protocol}[1]{\noindent\hrulefill\\\noindent{\bf {#1}}\small}{\normalsize\hrulefill}

%%%%%%%%%%%% Named References %%%%%%%%%%%%%%%%%%%%%

%
\newcommand{\namedref}[3]{\hyperref[#2:#3]{#1~\ref*{#2:#3}}}
%% if you don't like it, use this instead:
%\newcommand{\namedref}[3]{#1~\ref{#2:#3}}

\newcommand{\sectionref}[1]{\namedref{Section}{sec}{#1}}
\newcommand{\appendixref}[1]{\namedref{Appendix}{app}{#1}}
\newcommand{\theoremref}[1]{\namedref{Theorem}{thm}{#1}}
\newcommand{\definitionref}[1]{\namedref{Definition}{def}{#1}}
\newcommand{\corollaryref}[1]{\namedref{Corollary}{cor}{#1}}
\newcommand{\propositionref}[1]{\namedref{Proposition}{pro}{#1}}
\newcommand{\lemmaref}[1]{\namedref{Lemma}{lem}{#1}}
\newcommand{\claimref}[1]{\namedref{Claim}{clm}{#1}}
\newcommand{\figureref}[1]{\namedref{Figure}{fig}{#1}}
\newcommand{\tableref}[1]{\namedref{Table}{tab}{#1}}
\newcommand{\footnoteref}[1]{\namedref{Footnote}{foot}{#1}}
\newcommand{\equationref}[1]{\namedref{Equation}{eq}{#1}}



%% %% http://www.tug.org/TeXnik/mainFAQ.cgi?file=counter/counter#number
%% %%
%% \newcommand*{\numtodos}{0}
%% \makeatletter
%% \AtBeginDocument{%
%%   \AtEndDocument{%
%%     \immediate\write\@mainaux{%
%%       \string\gdef\string\numtodos{\number\value{todos}}%
%%     }%
%%   }%
%% }
%% \makeatother
%%
%%
%%
%% % Different font in captions
%% \newcommand{\captionfonts}{\small}
%%
%% \makeatletter  % Allow the use of @ in command names
%% \long\def\@makecaption#1#2{%
%%   \vskip\abovecaptionskip
%%   \sbox\@tempboxa{{\captionfonts #1: #2}}%
%%   \ifdim \wd\@tempboxa >\hsize
%%     {\captionfonts #1: #2\par}
%%   \else
%%     \hbox to\hsize{\hfil\box\@tempboxa\hfil}%
%%   \fi
%%   \vskip\belowcaptionskip}
%% \makeatother   % Cancel the effect of \makeatletter
%%
%% \fi


%%%%%%%% Handy Math Macros %%%%%%%%%%%%
\newcommand{\half}{\ensuremath{\nicefrac12}\xspace}
\newcommand{\xor}{\ensuremath{\oplus}\xspace}
\newcommand{\Xor}{\ensuremath{\bigoplus}\xspace}
\newcommand{\ceil}[1]{\ensuremath{\lceil{#1}\rceil}\xspace}
\newcommand{\floor}[1]{\ensuremath{\lfloor{#1}\rfloor}\xspace}
\newcommand{\from}{\leftarrow}
\newcommand{\gives}{\rightarrow}
\newcommand{\pr}[1]{\ensuremath{{\mathrm{Pr}}[#1]}}
\newcommand{\prr}[2]{\ensuremath{{\mathrm{Pr}_{#1}}[#2]}}
\newcommand{\prl}[2]{\ensuremath{{\underset{#1}{\mathrm{Pr}}}[#2]}}
\newcommand{\indist}{\ensuremath{\approx}}
\newcommand{\poly}{\ensuremath{\mathrm{poly}}\xspace}
\newcommand{\polylog}{\ensuremath{\mathrm{polylog}}\xspace}
\newcommand{\negl}{\ensuremath{\mathrm{negl}}\xspace}

\newcommand{\ZZ}{\ensuremath{\mathbb Z}\xspace}
\newcommand{\NN}{\ensuremath{\mathbb N}\xspace}
\newcommand{\FF}{\ensuremath{\mathbb{F}}\xspace}
\newcommand{\RR}{\ensuremath{\mathbb{R}}\xspace}
\newcommand{\set}[1]{\ensuremath{\{ #1 \}}\xspace}
\newcommand{\abs}[1]{\ensuremath{\left| #1\right|}\xspace}
\newcommand{\bits}{\ensuremath{\set{0,1}}\xspace}

\mathtoolsset{centercolon}
\newcommand{\eqdef}{\stackrel{\mbox{\tiny def}}{{=}}}

%%%%%%%%%%%%%%%%% End Generic Stuff %%%%%%%%%%%%%%%%%%%%%%%


%%%%%%%%%%%%%%%%% Macros for Nash paper %%%%%%%%%%%%%%%%%%%%%%

\newcommand{\LitSet}{{\ensuremath{{\text{LitSet}}}}\xspace}
\newcommand{\Index}{{\ensuremath{{\text{Index}}}}\xspace}

%%%%%%%%%%%%%%%%% Macros for Nash paper %%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%% Macros for this paper %%%%%%%%%%%%%%%%%%%%%%
\newcommand{\hatC}{\ensuremath{\hat{C}}\xspace}
\newcommand{\hatK}{\ensuremath{\hat{K}}\xspace}
\newcommand{\hatKK}{\ensuremath{\tilde{K}}\xspace}
\newcommand{\hatX}{\ensuremath{\hat{X}}\xspace}
\newcommand{\hatXX}{\ensuremath{\tilde{X}}\xspace}
\newcommand{\hatd}{\ensuremath{\hat{d}}\xspace}
\newcommand{\haty}{\ensuremath{\hat{y}}\xspace}
\newcommand{\Gb}{{\ensuremath{{\text{Gb}}}}\xspace}
\newcommand{\Gbof}[1]{\ensuremath{{\Gb_{#1}}}\xspace}
\newcommand{\Eval}{{\ensuremath{{\text{Eval}}}}\xspace}
\newcommand{\Evalof}[1]{\ensuremath{{\Eval_{#1}}}\xspace}

\newcommand{\In}{{\ensuremath{{\text{In}}}}\xspace}
\newcommand{\Sim}{{\ensuremath{{\text{Sim}}}}\xspace}
\newcommand{\Simof}[1]{\ensuremath{{\Sim_{#1}}}\xspace}
\newcommand{\cind}{\ensuremath{\overset{c}{\approx}}\xspace}
\newcommand{\cindx}[1]{\ensuremath{\overset{c,#1}{\approx}}\xspace}
\newcommand{\ncind}{\ensuremath{\overset{c}{\not\approx}}\xspace}
\newcommand{\sind}{\ensuremath{\overset{s}{\approx}}\xspace}
\newcommand{\sindx}[1]{\ensuremath{\overset{s,#1}{\approx}}\xspace}

\newcommand{\DD}[1]{\ensuremath{{\Psi_{#1}}}\xspace}
\newcommand{\DDK}{\ensuremath{{\DD{K}}}\xspace}
\newcommand{\DDM}{\ensuremath{{\DD{M}}}\xspace}
\newcommand{\DDC}{\ensuremath{{\DD{C}}}\xspace}

\newcommand{\Gen}{\entity{Gen}}
\newcommand{\Enc}{\entity{Enc}}
\newcommand{\Dec}{\entity{Dec}}
\newcommand{\Genof}[1]{\ensuremath{{\Gen_{#1}}}\xspace}
\newcommand{\Encof}[1]{\ensuremath{{\Enc_{#1}}}\xspace}
\newcommand{\Decof}[1]{\ensuremath{{\Dec_{#1}}}\xspace}
%\newcommand{\Encr}{{\ensuremath{{\Enc.ran}}}\xspace}
\newcommand{\Encr}{\entity{Ran}}
\newcommand{\Encrof}[1]{{\ensuremath{{\Encr_{#1}}}}\xspace}

\newcommand{\inr}{\ensuremath{{\in_{R}}}\xspace}
\newcommand{\PS}{\fname{PackedShare}}
\newcommand{\SR}{\fname{PackedShareRct}}
\newcommand{\BitDecomp}{\fname{BitDecomp}}
\newcommand{\U}{\entity{U}} %Uniform Distribution
\newcommand{\stage}[1]{{\ensuremath{{\text{stage}_{#1}}}}\xspace}
\newcommand{\mybox}[3]{\ensuremath{{\boxed{#1}}^{#2}_{#3}}\xspace}


%%%%%%%%%%%%%%%%% Macros for MPC and this paper %%%%%%%%%%%%%%%%%%%

\newcommand{\functionality}[1]{\ensuremath{{\mathcal #1}}\xspace}
\newcommand{\keyword}[1]{\ensuremath{{\text{\sc #1}}}\xspace}
\newcommand{\command}[1]{\ensuremath{{\text{\sf #1}}}\xspace}
\newcommand{\entity}[1]{\ensuremath{{\text{\sf #1}}}\xspace}
\newcommand{\fname}[1]{{\text{\sf #1}}\xspace}
\newcommand{\xfname}[1]{\ensuremath{\widetilde{\fname{#1}}}\xspace}

\newcommand{\compclass}[1]{\ensuremath{\text{\bf{#1}}}\xspace}
\newcommand{\NC}[1]{\ensuremath{\compclass{NC}^{#1}}\xspace} % use as \NC0, \NC1 etc.


\newcommand{\codeof}[1]{\ensuremath{\langle{#1}\rangle}\xspace}

% \newcommand{\secpar}{\ensuremath{\kappa}\xspace}

% state and message
%\newcommand{\state}{\ensuremath{\sigma}\xspace}
\newcommand{\msg}{\ensuremath{\mu}\xspace}
\newcommand{\statespace}{\ensuremath{\Sigma}\xspace}
\newcommand{\msgspace}{\ensuremath{M}\xspace}
\newcommand{\secretspace}{\ensuremath{\mathcal{M}}\xspace}

% experiment def
\newcommand{\static}{\ensuremath{\security{static}}\xspace}
\newcommand{\adp}{\ensuremath{\security{adapt1}}\xspace}
\newcommand{\fulladp}{\ensuremath{\security{adapt2}}\xspace}

\newcommand{\Sem}{\ensuremath{\security{SS}}\xspace} %Semantic Secure
\newcommand{\MI}{\ensuremath{\security{MI}}\xspace} %Message Indistinguishability
\newcommand{\Inc}{\ensuremath{\security{Inc}}\xspace} %Incompressible
\newcommand{\IND}[1]{\ensuremath{\text{\security{IND}-{#1}}}\xspace}
\newcommand{\SIM}[1]{\ensuremath{\text{\security{SIM}-{#1}}}\xspace}
\newcommand{\PRG}{\ensuremath{\security{PRG}}\xspace}
\newcommand{\PRP}{\ensuremath{\security{PRP}}\xspace}
\newcommand{\OWF}{\ensuremath{\security{PRP}}\xspace}
%\newcommand{\stat}{\ensuremath{\text{state}}\xspace}

\newcommand{\Exp}{\ensuremath{\textbf{Exp}}\xspace}
\newcommand{\Expof}[1]{\ensuremath{{\Exp^{#1}}}\xspace}
\newcommand{\Advoff}[2]{\ensuremath{{\adv^{#1}_{#2}}}\xspace}
\newcommand{\Hybrid}[1]{\ensuremath{\textbf{Hybrid{#1}}}\xspace}

% security definitions
\newcommand{\security}[1]{{\ensuremath{{\text{\sf #1}}}}\xspace}
\newcommand{\secure}{\security{secure}}

\newcommand{\sh}{\ensuremath{\security{sh}}\xspace}
\newcommand{\act}{\ensuremath{\security{full}}\xspace}
\newcommand{\id}{\ensuremath{\security{id}}\xspace}
\newcommand{\xid}[1]{\ensuremath{{{#1}\security{-id}}}\xspace}
\newcommand{\xxid}[1]{\ensuremath{{\security{id}_{#1}}}\xspace}
\newcommand{\xidBC}[1]{\ensuremath{{{#1}\security{-id/\BC}}}\xspace}
\newcommand{\xxidBC}[2]{\ensuremath{{{#1}\security{-\xxid{#2}/\BC}}}\xspace}
\newcommand{\idxx}[2]{\ensuremath{{{#1}\security{-id}_{#2}}}\xspace}
\newcommand{\twoid}{\ensuremath{\xxid{\half}}\xspace}
\newcommand{\thetaid}{\ensuremath{\xxid\theta}\xspace}
\newcommand{\idalpha}{\ensuremath{\xxid\alpha}\xspace}

\newcommand{\xsecure}[1]{\ensuremath{{{#1}\security{-secure}}}\xspace}
\newcommand{\xact}[1]{\ensuremath{{{#1}\security{-full}}}\xspace}
\newcommand{\xactfull}[1]{\ensuremath{\xact{#1}}\xspace}
\newcommand{\xsh}[1]{\ensuremath{{{#1}\security{-sh}}}\xspace}
\newcommand{\xabort}[1]{\ensuremath{{{#1}\security{-abort}}}\xspace}
\newcommand{\xactBC}[1]{\ensuremath{{{#1}\security{-full/\BC}}}\xspace}


\newcommand{\alphash}{{\xsh\alpha}}
\newcommand{\betash}{{\xsh\beta}}
\newcommand{\alphaact}{{\xact\alpha}}
\newcommand{\alphaactBC}{{\xactBC\alpha}}
\newcommand{\betaact}{{\xact\beta}}
\newcommand{\alphashstar}{{\xsh\alpha^*}}

\newcommand{\alphaid}{\ensuremath{\xid\alpha}\xspace}
\newcommand{\alphaidBC}{\ensuremath{\xidBC\alpha}\xspace}
\newcommand{\alphaxid}[1]{\ensuremath{\xxid\alpha{#1}}\xspace}
\newcommand{\alphaxidBC}[1]{\ensuremath{\xxidBC\alpha{#1}}\xspace}
\newcommand{\alphaabort}{\ensuremath{\xabort\alpha}\xspace}

\newcommand{\shot}{\ensuremath{\security{sh/}\OT}\xspace}
\newcommand{\actot}{\ensuremath{\security{full/}\OT}\xspace}
\newcommand{\shppt}{\ensuremath{\security{sh-ppt}}\xspace}
\newcommand{\actpptuc}{\ensuremath{\security{full-ppt-uc}}\xspace} % uc security
\newcommand{\actpptsa}{\ensuremath{\security{full-ppt-sa}}\xspace} % standalone security
\newcommand{\actpptid}{\ensuremath{\security{full-ppt-sa-id}}\xspace}

\newcommand{\alphaactfull}{\alphaact}
\newcommand{\betaactfull}{\betaact}

\newcommand{\funqual}[2]{\ensuremath{{#1}^{\langle{#2}\rangle}}\xspace}
\newcommand{\funid}[1]{\ensuremath{\funqual{#1}{\thetaid}}\xspace}
\newcommand{\fid}[2]{\ensuremath{\funqual{#1}{\xxid{#2}}}\xspace}
\newcommand{\funabort}[1]{\ensuremath{\funqual{#1}{\abort}}\xspace}
\newcommand{\level}{level\xspace}

\newcommand{\BBT}{\ensuremath{\text{BBT}}\xspace}

\newcommand{\G}{\ensuremath{{\mathcal G}}\xspace}
\newcommand{\F}{\ensuremath{{\mathcal F}}\xspace}
\newcommand{\Sec}{\ensuremath{\Lambda}\xspace}
\newcommand{\Secof}[2]{\ensuremath{{\Sec_{#1}^{#2}}}\xspace}
\newcommand{\Secoff}[1]{\ensuremath{{\Sec_{#1}}}\xspace}
\newcommand{\Secofff}[1]{\ensuremath{{\Sec'_{#1}}}\xspace}
\newcommand{\XSec}{\ensuremath{{\widehat{\Lambda}}}\xspace}
\newcommand{\XSecof}[2]{\ensuremath{{\XSec_{#1}^{#2}}}\xspace}
\renewcommand{\P}{\ensuremath{\mathcal P}\xspace}
\newcommand{\Fall}{\ensuremath{{\mathcal F}^*}\xspace}
\newcommand{\Frnds}{\ensuremath{{\mathcal F}^+}\xspace}
\newcommand{\Fzk}{\ensuremath{{\mathcal F}_{\mathrm{ZK}}}\xspace}
\newcommand{\Fcom}{\ensuremath{{\mathcal F}_{\mathrm{Com}}}\xspace}
\newcommand{\Farith}{\ensuremath{{\mathcal F}_{\mathrm{arith}}}\xspace}
\newcommand{\W}{\ensuremath{{\mathcal W}}\xspace}

\newcommand{\compSecof}[3]{\ensuremath{{#1}\operatorname{-}{\Secof{#2}{#3}}}\xspace}
\newcommand{\compSecoff}[2]{\compSecof{#1}{#2}{}}

\newcommand{\xcompSecof}[3]{\ensuremath{(#1)\text{\texttildelow}{\Secof{#2}{#3}}}\xspace}
\newcommand{\xcompSecoff}[2]{\xcompSecof{#1}{#2}{}}

\newcommand{\compSecofxa}[3]{\compSecof{(#1)}{#2}{#3}}
\newcommand{\compSecoffxa}[2]{\compSecoff{(#1)}{#2}}

\newcommand{\compSecofxb}[3]{\compSecof{\langle#1\rangle}{#2}{#3}}
\newcommand{\compSecoffxb}[2]{\compSecoff{\langle#1\rangle}{#2}}

\newcommand{\ECSSShare}{\ensuremath{\mathrm{ECSS-Share}}\xspace}
\newcommand{\ECSSReconstruct}{\ensuremath{\mathrm{ECSS-Reconstruct}}\xspace}
\newcommand{\TIPS}[1]{\ensuremath{T^{\mathrm{IPS}}_{#1}}\xspace}
\newcommand{\coreIPS}{\ensuremath{{\mathrm{IPS}}_{\mathrm{core}}}\xspace}
\newcommand{\WgenIPS}{\ensuremath{{\mathrm{IPS}}_{\mathrm{WL}}}\xspace}
\newcommand{\wIPS}{\ensuremath{w_{\mathrm{IPS}}}\xspace}

%\newcommand{\FxRabOT}{\ensuremath{\F_{\xRabOT}}\xspace}
\newcommand{\FxRabOT}{\ensuremath{\xRabOT}\xspace}
\newcommand{\PxRabOT}{\ensuremath{\pi_{\xRabOT}}\xspace}
\newcommand{\AMDlite}{\ensuremath{\mathsf{AMDlite}}\xspace}

\newcommand{\share}{\command{share}}
\newcommand{\reconstruct}{\command{reconstruct}}
\newcommand{\corrupt}{\command{corrupt}}
\newcommand{\abort}{\command{abort}}
\newcommand{\erased}{\command{erased}}
\newcommand{\corruptsession}{\command{corruptsession}}
\newcommand{\default}{\command{default}}
\newcommand{\full}{\command{full}}

\newcommand{\layer}{\command{layer}}

\newcommand{\ideal}{\keyword{ideal}}
\newcommand{\real}{\keyword{real}}
\newcommand{\mac}{\keyword{mac}}

\newcommand{\env}{\entity{Env}}
\newcommand{\adv}{\entity{Adv}}
\newcommand{\simu}{\entity{Sim}}
\newcommand{\pad}{\entity{Pad}}


\newcommand{\pout}{\ensuremath{p_{\mathrm{out}}}\xspace}
\newcommand{\qout}{\ensuremath{q_{\mathrm{out}}}\xspace}
\newcommand{\pin}{\ensuremath{p_{\mathrm{in}}}\xspace}
\newcommand{\qin}{\ensuremath{q_{\mathrm{in}}}\xspace}
\newcommand{\rin}{\ensuremath{r_{\mathrm{in}}}\xspace}

\newcommand{\degree}{\ensuremath{\bar{D}}\xspace}

\newcommand{\OT}{\fname{OT}}
\newcommand{\sOT}{\fname{string-OT}}
\newcommand{\sOTell}{\fname{string-OT$[\ell]$}}
\newcommand{\OLE}{\fname{OLE}}
\newcommand{\BC}{\fname{BC}}
\newcommand{\COM}{\fname{COM}}

\newcommand{\consistent}{\command{consistent}}
\newcommand{\xRabOT}{\xfname{OT}}

\newcommand{\Size}{\command{size}}
\newcommand{\Depth}{\command{depth}}
\newcommand{\Width}{\command{width}}
\newcommand{\Widthx}[2]{\ensuremath{\Width_{#1}({#2})}\xspace}
\newcommand{\D}{\command{D}}
\newcommand{\Din}{\ensuremath{\D_\mathrm{in}}\xspace}
\newcommand{\Dout}{\ensuremath{\D_\mathrm{out}}\xspace}

%%%%%%%%%%
% TikZ style
\tikzset{%
auto,
 pnode/.style = {rectangle,draw,fill=white,rounded corners=5pt,minimum size=1cm},
 bnode/.style = {rectangle,draw,ultra thick,gray,fill=white,minimum size=1cm}
}

\pgfdeclarelayer{bg}    % declare background layer
\pgfsetlayers{bg,main}  % set the order of the layers (main is the standard layer)


